Discovery of distant high luminosity infrared galaxies

We have developed a method for selecting the most luminous galaxies detected by IRAS based on their extreme values of R, the ratio of 60 micron and B-band luminosity. These objects have optical counterparts that are close to or below the limits of Schmidt surveys. We have tested our method on a 1079 deg^2 region of sky, where we have selected a sample of IRAS sources with 60 micron flux densities greater than 0.2 Jy, corresponding to a redshift limit z~1 for objects with far-IR luminosities of 10^{13} L_sun. Optical identifications for these were obtained from the UK Schmidt Telescope plates, using the likelihood ratio method. Optical spectroscopy has been carried out to reliably identify and measure the redshifts of six objects with very faint optical counterparts, which are the only objects with R>100 in the sample. One object is a hyperluminous infrared galaxy (HyLIG) at z=0.834. Of the remaining, fainter objects, five are ultraluminous infrared galaxies (ULIGs) with a mean redshift of 0.45, higher than the highest known redshift of any non-hyperluminous ULIG prior to this study. High excitation lines reveal the presence of an active nucleus in the HyLIG, just as in the other known infrared-selected HyLIGs. In contrast, no high excitation lines are found in the non-hyperluminous ULIGs. We discuss the implications of our results for the number density of HyLIGs at z<1 and for the evolution of the infrared galaxy population out to this redshift, and show that substantial evolution is indicated. Our selection method is robust against the presence of gravitational lensing if the optical and infrared magnification factors are similar, and we suggest a way of using it to select candidate gravitationally lensed infrared galaxies.

==> hyphens.tex <==
\hyphenation{ASTRON}                    % how to (not) break these words
\hyphenation{cloud-let cloud-lets}
\hyphenation{HVABG}
\hyphenation{MNRAS}
\hyphenation{Peim-bert}
\hyphenation{Schloerb}
\endinput


==> molec.tex <==
%--------------- molecules and molecular ions --------------------------------
%

\def\mbox{\hbox}           % for compatibility of TeX and LaTeX use 

\def\CO#1{\ifnum#1=0                    % CO isotopes
           \ifmmode \mbox{\rm CO}
           \else {\rm CO}
           \fi
          \else
           \ifnum#1<15
            \ifmmode ^{#1}\mbox{\rm CO}
            \else $^{#1}${\rm CO}
            \fi
           \else
            \ifmmode \mbox{\rm C}^{#1}\mbox{\rm O}
            \else {\rm C}$^{#1}${\rm O}
            \fi
           \fi
          \fi}

\def\COp{\ifmmode \mbox{\rm CO}^+           %   +
         \else {\rm CO}$^+$                 % CO
         \fi}

\def\CS#1{\ifnum#1=0                    % CS isotopes
           \ifmmode \mbox{\rm CS}
           \else {\rm CS}
           \fi
          \else
           \ifnum#1<15
            \ifmmode ^{#1}\mbox{\rm CS}
            \else $^{#1}${\rm CS}
            \fi
           \else
            \ifmmode \mbox{\rm C}^{#1}\mbox{\rm S}
            \else {\rm C}$^{#1}${\rm S}
            \fi
           \fi
          \fi}

\def\HCOp{\ifmmode \mbox{\rm HCO}^+          %    +
          \else {\rm HCO}$^+$                % HCO
          \fi}
                                               %  +
\def\Hthreep{\ifmmode \mbox{\rm H}_3^+         % H
             \else {\rm H}$_3^+$               %  3
             \fi}

\def\Htwo{\ifmmode \mbox{\rm H}_2              % H
          \else {\rm H}$_2$                    %  2
          \fi}

\def\HtwoO{\ifmmode \mbox{\rm H}_2\mbox{\rm O} % H O
           \else {\rm H}$_2${\rm O}            %  2
           \fi}

%
%---------------------- atoms and atomic ions ---------------------------------
%

\def\ion#1#2{\ifmmode \mbox{{\rm #1}}\,\mbox{{\sc #2}} % generic ion
        \else {\rm #1}$\,${\sc #2}
        \fi}
\def\HI{\ion{H}{i}}
\def\HII{\ion{H}{ii}}

%
%-------------------- hydrogen recombination lines ---------------------------
%

\def\rec#1#2{\if#2a                            % generic
              \ifmmode \mbox{{\rm #1}}\alpha   % recombination line
              \else {\rm #1}$\alpha$
              \fi
             \fi
             \if#2b
              \ifmmode \mbox{{\rm #1}}\beta
              \else {\rm #1}$\beta$
              \fi
             \fi
             \if#2g
              \ifmmode \mbox{{\rm #1}}\gamma
              \else {\rm #1}$\gamma$
              \fi
             \fi}

\def\Lya{\rec{Ly}{a}}                          % Lyman alpha
\def\Ha{\rec{H}{a}}                            % H alpha
\def\Brg{\rec{Br}{g}}                          % Brackett gamma

\endinput


==> refs.tex <==
%..............................................................................
%
%             This is    r e f s . t e x
%
% A LaTeX file for keeping tracks of references to figures, sections,
% tables and equations.
%
% Latest update: Paul van der Werf 21-Mar-1994
%
%..............................................................................

\newcommand{\tabref}[1]{Table~\protect\ref{#1}}
\newcommand{\figref}[1]{Fig.~\protect\ref{#1}}
\newcommand{\figrefbare}[1]{\protect\ref{#1}}
\newcommand{\figrefs}[1]{Figs.~\protect\ref{#1}}
\newcommand{\figsref}[2]{Figs.~\protect\ref{#1}--\protect\ref{#2}}
\newcommand{\twofigsref}[2]{Figs.~\protect\ref{#1} and~\protect\ref{#2}}
\newcommand{\eqref}[1]{Eq.~$\left(\protect\ref{#1}\right)$}
\newcommand{\eqsref}[2]{Eqs.~$\left(\protect\ref{#1}\right)$--$\left(\protect\ref{#2}\right)$}
\newcommand{\secref}[1]{Sect.~\protect\ref{#1}}
\newcommand{\secsref}[2]{Sects.~\protect\ref{#1}--\protect\ref{#2}}
\newcommand{\twosecsref}[2]{Sects.~\protect\ref{#1} and~\protect\ref{#2}}

% upper case versions to begin sentences: 

\newcommand{\Tabref}[1]{\tabref{#1}}
\newcommand{\Figref}[1]{Figure~\protect\ref{#1}}
\newcommand{\Figrefs}[1]{Figures~\protect\refs{#1}}
\newcommand{\Figsref}[2]{Figures~\protect\ref{#1}--\protect\ref{#2}}
\newcommand{\Eqref}[1]{Equation~(\protect\ref{#1})}
\newcommand{\Eqsref}[2]{Equations~(\protect\ref{#1})--(\protect\ref{#2})}
\newcommand{\Secref}[1]{Section~\protect\ref{#1}}

\endinput


==> symbols.tex <==
\def\mbox{\hbox}           % for compatibility of TeX and LaTeX use

%------------------ degrees, magnitudes, RA, Dec etc -------------------------
%

\def\deg{\ifmmode ^\circ                % degrees symbol
         \else $^\circ$
         \fi
         \hskip -0.1truecm}
\def\degd#1.#2{                         % degrees over decimal point
                                        % syntax: \degd 4.3 or \degd 4.{34}
               \ifmmode {#1^{\hskip 0.05em\circ}\hskip-0.42em.\hskip0.08em#2}
               \else {#1$^{\hskip 0.05em\circ}\hskip-0.42em.\hskip0.08em$#2}
               \fi
              }
\def\mind#1.#2{                         % minutes over decimal point
                                        % syntax: \mind 4.3
               \ifmmode {#1^{\hskip 0.05em\prime}\hskip-0.35em.\hskip0.05em#2}
               \else {#1$^{\hskip 0.05em\prime}\hskip-0.35em.\hskip0.05em$#2}
               \fi
              }
\def\secd#1.#2{                         % seconds over decimal point
                                        % syntax: \secd 4.3
               \ifmmode {#1^{\prime\prime}\hskip-0.46em.\hskip0.12em#2}
               \else {#1$^{\prime\prime}\hskip-0.46em.\hskip0.12em$#2}
               \fi
              }
\def\timsecd#1.#2{                      % time seconds over decimal point
                                        % syntax: \timsecd 4.3
                  \ifmmode {#1^{\rm s}\hskip-0.39em.\hskip0.08em#2}
                  \else {$#1^{\rm s}\hskip-0.39em.\hskip0.08em#2$}
                  \fi
                 }
\def\hms#1h#2m#3s{                      % hms format (for RA)
                                        % syntax: \hms 12h34m45s
                  \relax
                  \ifmmode #1^{\rm h}\,#2^{\rm m}\,#3^{\rm s}
                  \else \hbox{$#1^{\rm h}\,#2^{\rm m}\,#3^{\rm s}$}
                  \fi
                 }
\def\dms#1d#2m#3s{                      % dms format (for Dec)
                                        % syntax: \dms 12d14m45s
                  \relax
                  \ifmmode #1^\circ\,#2^{\prime}\,#3^{\prime\prime}
                  \else \hbox{$#1^\circ\,#2^{\prime}\,#3^{\prime\prime}$}
                  \fi
                 }
\def\dmsd#1d#2m#3.#4s{                  % dms format with decimal point (Dec)
                                        % syntax: \dmsd 12d13m34.5s
                      \relax
                      \ifmmode #1^\circ\,#2^{\prime}\,#3^{\prime\prime}
                               \hskip-0.46em.\hskip0.12em#4
                      \else \hbox{$#1^\circ\,#2^{\prime}\,#3^{\prime\prime}
                            \hskip-0.46em.\hskip0.12em#4$}
                      \fi
                     }
\def\hm#1h#2m{                          % hm format (for RA)
                                        % syntax: \hm 12h13m
              \relax
              \ifmmode #1^{rm h}\,#2^{\rm m}
              \else \hbox{$#1^{\rm h}\,#2^{\rm m}$}
              \fi
             }
\def\dm#1d#2m{                          % dm format (for Dec)
                                        % syntax: \dm 12d13m
              \relax
              \ifmmode #1^\circ\,#2^{\prime}
              \else \hbox{$#1^\circ\,#2^{\prime}$}
              \fi
             }
\def\hmsd#1h#2m#3.#4s{                  % hms format with decimal point (RA)
                                        % syntax: \hmsd 12h13m34.5s
                      \relax
                      \ifmmode #1^{\rm h}\,#2^{\rm m}\,#3^{\rm s}
                               \hskip-0.39em.\hskip0.08em#4
                      \else \hbox{$#1^{\rm h}\,#2^{\rm m}\,#3^{\rm s}
                            \hskip-0.39em.\hskip0.08em#4$}
                      \fi
                     }
\def\hmd#1h#2.#3m{                  % hm format with decimal point (RA)
                                    % syntax: \hmd 12h13.6m
                  \relax
                  \ifmmode #1^{\rm h}\,#2^{\rm m}
                           \hskip-0.55em.\hskip0.22em#3
                  \else \hbox{$#1^{\rm h}\,#2^{\rm m}
                        \hskip-0.55em.\hskip0.22em#3$}
                  \fi
                 }
\def\mg{\relax                          % magnitudes symbol
        \ifmmode ^{\rm m}
        \else $^{\rm m}$
        \fi
       }
\def\mgd#1.#2{                          % magnitudes over decimal point
                                        % syntax: \mgd 4.3
              \relax
              \ifmmode #1^{\rm m}
                       \hskip-0.55em.\hskip0.22em#2
              \else \hbox{#1$^{\rm m}
                    \hskip-0.55em.\hskip0.22em$#2}
              \fi
             }

%
%-------------------- math symbols --------------------------------------------
%

\def\la{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\def\ga{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}

%
%--------------------------- units -------------------------------------------
% use: e.g. $15\kms$
%

\def\unitspace{\,}                      % space to be used with units

\def\un#1{\ifmmode \unitspace\mbox{\rm #1} % generic unit
          \else $\unitspace$#1
          \fi}
\def\pun#1#2{\ifmmode \unitspace\mbox{\rm #1}^{#2} % generic unit with a power
             \else $\unitspace$#1$^{#2}$
             \fi}

\def\es{\un{erg}\psec}                %      -1
                                      % erg s
\def\esc{\es\pcmsqu}                  %      -1 -2
                                      % erg s cm
\def\escmum{\esc\mum^{-1}}            %      -1 -2  -1
                                      % erg s cm  mu
\def\escs{\esc\pun{sr}{-1}}           %      -1 -2 -1
                                      % erg s cm sr
\def\escsm{\escs\mum^{-1}}            %      -1 -2 -1 -1
                                      % erg s cm sr mu
\def\GHz{\un{GHz}}                    % GHz
\def\kms{\un{km}\pun{s}{-1}}          %     -1
                                      % km s
\def\Lsun{\ifmmode \un{L}_{\odot}     % solar luminosity
          \else $\un{L}_{\odot}$
          \fi}
\def\Msun{\ifmmode \un{M}_{\odot}     % solar mass
          \else $\un{M}_{\odot}$
          \fi}
\def\mum{\ifmmode \unitspace\mu\mbox{\rm m} % micron
         \else $\unitspace\mu$m
         \fi}
\def\pcmcub{\pun{cm}{-3}}             %   -3
                                      % cm
\def\pcmsqu{\pun{cm}{-2}} %   -2
                          % cm
\def\pyr{\pun{yr}{-1}}    %   -1
                          % yr
\def\psec{\pun{s}{-1}}    %  -1
                          % s

%
%-------------------------- quantities ---------------------------------------
%

\def\Bp{\relax                            % B
        \ifmmode B_{||}                   %  ||
        \else $B_{||}$
        \fi}
\def\Bt{\relax                            % B
        \ifmmode B\!_{\perp}              %  |
        \else $B\!_{\perp}$               %  -
        \fi}
\def\Gcr{\relax                           % Gamma
         \ifmmode \Gamma\!_{\rm cr}       %      cr
         \else $\Gamma\!_{\rm cr}$
         \fi}
\def\ICII{\relax                          % I
          \ifmmode I_{[\CII]}             %  [C II]
          \else $I_{[\CII]}$
          \fi}
\def\LHtwo{\relax                                 % L
           \ifmmode L_{\mbox{\rm\scriptsize H}_2} %  H
           \else $L_{\mbox{\rm\scriptsize H}_2}$  %   2
           \fi}
\def\LLya{\relax                          % L
          \ifmmode L_{{\rm Ly}\,\alpha}   %  Ly alpha
          \else $L_{{\rm Ly}\,\alpha}$
          \fi}
\def\MHtwo{\relax                                 % M
           \ifmmode M_{\mbox{\rm\scriptsize H}_2} %  H
           \else $M_{\mbox{\rm\scriptsize H}_2}$  %   2
           \fi}
\def\MHtwodot{\relax                                       % .
              \ifmmode \dot{M}_{\mbox{\rm\scriptsize H}_2} % M
              \else $\dot{M}_{\mbox{\rm\scriptsize H}_2}$  %  H
              \fi}                                         %   2
\def\Mstardot{\relax                      % .
              \ifmmode \dot{M}_{\ast}     % M
              \else $\dot{M}_{\ast}$      %  *
              \fi}
\def\nHI{\relax                                      % n
         \ifmmode n_{\mbox{\scriptsize\rm H\,\sc I}} %  HI
         \else $n_{\mbox{\scriptsize\rm H\,\sc I}}$
         \fi}
\def\nHtwo{\relax                                % n
           \ifmmode n_{{\mbox{\scriptsize H}}_2} %  H
           \else $n_{{\mbox{\scriptsize H}}_2}$  %   2
           \fi}

%
%------------------ source designations -------------------------
%

\def\sou#1#2{\relax                       % source designations
             \ifmmode {\rm #1}\,{\rm #2}  % e.g. \sou{Arp}{220}
             \else #1$\,$#2
             \fi}

\def\NGC#1{\sou{NGC}{#1}}                % NGC number

%
%------------------- generic quantity symbols ------------------
%

\def\qu#1#2{\relax                          % quantity symbols
            \ifmmode #1_{\rm #2}            % e.g. \qu{L}{FIR}
            \else $#1_{\rm #2}$
            \fi}

\endinput

